What can Neural Referential Form Selectors Learn?

Despite achieving encouraging results, neural Referring Expression Generation models are often thought to lack transparency. We probed neural Referential Form Selection (RFS) models to find out to what extent the linguistic features influencing the RE form are learnt and captured by state-of-the-art RFS models. The results of 8 probing tasks show that all the defined features were learnt to some extent. The probing tasks pertaining to referential status and syntactic position exhibited the highest performance. The lowest performance was achieved by the probing models designed to predict discourse structure properties beyond the sentence level.

==> tab/classifier_4.tex <==
\begin{table}[t!]
\small
\centering
\begin{tabular}{llccc}
\toprule
Model & Precision & Recall & F1 \\ \midrule
\texttt{CatBoost} & 52.26 (-) & 49.51 (-) & 46.88 (-) \\ \midrule
\texttt{c-RNN} & 68.79 (2.63) & 62.95 (1.68) & 64.96 (1.78) \\
\texttt{ +Glove} & 69.10 (3.90) & 63.90 (1.94) & 65.40 (2.10) \\
\texttt{ +BERT} \\
\texttt{ConATT} & 67.42 (2.20) & 62.39 (1.93) & 64.07 (1.88) \\
\texttt{ +Glove} & 65.98 (3.60) & 62.49 (1.97) & 63.67 (2.13) \\
\bottomrule
\end{tabular}
\caption{4 way classification Results on \textsc{webnlg} corpus.}
\label{tab:cls1}
\end{table}

==> tab/cm.tex <==
%catboost 2-way ConfMat

%               Reference
% Prediction      nonpronominal pronominal
%   nonpronominal          8965        145
%   pronominal              133        401


% catboost 3-way ConfMat

%              Reference
% Prediction    description name pronoun
%   description         728  316      52
%   name               1488 6372      52
%   pronoun             109   85     442

% catboost 4-way ConfMat

%               Reference
% Prediction      demonstrative description name pronoun
%   demonstrative             0           1    1       0
%   description              13         708  320      49
%   name                     19        1485 6373      50
%   pronoun                   8          91   79     447



% ##############  XGBooost results #############################

% 2-way ContMat

%               Reference
% Prediction      nonpronominal pronominal
%   nonpronominal          8978        181
%   pronominal              120        365


% 3-way ConfMax

%              Reference
% Prediction    description name pronoun
%   description         766  400      41
%   name               1444 6293      58
%   pronoun             115   80     447


% 4-way ConfMat

%               Reference
% Prediction      demonstrative description name pronoun
%   demonstrative             0           0    3       0
%   description              13         766  381      53
%   name                     19        1430 6306      49
%   pronoun                   8          89   83     444

==> tab/permutation_loss.tex <==
%2-way

%       variable mean_dropout_loss   label
% 1  _full_model_        0.02151863 xgboost
% 2        LocPro        0.02142733 xgboost
% 3       DistAnt        0.02335650 xgboost
% 4        IntRef        0.02402197 xgboost
% 5       MetaPro        0.02750374 xgboost
% 6       SenStat        0.02861941 xgboost
% 7        GloPro        0.03409244 xgboost
% 8           Syn        0.05012054 xgboost
% 9       DisStat        0.18782165 xgboost
% 10   _baseline_        0.47608103 xgboost


%3-way

%       variable mean_dropout_loss   label
% 1  _full_model_          583.8932 xgboost
% 2        IntRef          593.1987 xgboost
% 3        LocPro          595.7991 xgboost
% 4       DistAnt          599.0068 xgboost
% 5       SenStat          609.7033 xgboost
% 6        GloPro          620.0118 xgboost
% 7       MetaPro          626.1795 xgboost
% 8           Syn          654.2421 xgboost
% 9       DisStat          906.1781 xgboost
% 10   _baseline_         1079.0828 xgboost

%4-way 

%       variable mean_dropout_loss   label
% 1  _full_model_          0.000000 xgboost
% 2        LocPro          1.874938 xgboost
% 3        IntRef         14.347703 xgboost
% 4       DistAnt         17.114284 xgboost
% 5       SenStat         27.267791 xgboost
% 6        GloPro         40.674354 xgboost
% 7       MetaPro         43.473038 xgboost
% 8           Syn         73.176468 xgboost
% 9       DisStat        352.185883 xgboost
% 10   _baseline_        514.187626 xgboost


